Map-Aware Human Pose Prediction for Robot Follow-Ahead

In the robot follow-ahead task, a mobile robot is tasked to maintain its relative position in front of a moving human actor while keeping the actor in sight. To accomplish this task, it is important that the robot understand the full 3D pose of the human (since the head orientation can be different than the torso) and predict future human poses so as to plan accordingly. This prediction task is especially tricky in a complex environment with junctions and multiple corridors. In this work, we address the problem of forecasting the full 3D trajectory of a human in such environments. Our main insight is to show that one can first predict the 2D trajectory and then estimate the full 3D trajectory by conditioning the estimator on the predicted 2D trajectory. With this approach, we achieve results comparable or better than the state-of-the-art methods three times faster. As part of our contribution, we present a new dataset where, in contrast to existing datasets, the human motion is in a much larger area than a single room. We also present a complete robot system that integrates our human pose forecasting network on the mobile robot to enable real-time robot follow-ahead and present results from real-world experiments in multiple buildings on campus. Our project page, including supplementary material and videos, can be found at: https://qingyuan-jiang.github.io/iros2024_poseForecasting/

==> sections/acknowledgment.tex <==

% The authors would like to thank Ishan Shetty and all members of the Robotic Sensor Network Lab for their support. 
This work is supported by the NSF NRI Grant \#2022894.


==> sections/limitation.tex <==

In this section, we would like to provide a few limitations we face and find intractable. 
% From the method perspective, the current method cannot guarantee time consistency and is difficult to deal with T-conjunctions.
All failed cases end with the robot being unable to respond to the turn appropriately and the human walking too close to the robot such that the rear camera can only catch a limited part of the body pose and cannot predict. 
The algorithm cannot handle T-junction properly as it does not guarantee consistency over time.

Meanwhile, we would like to highlight that the planning algorithm for this robot follow-ahead problem is non-trivial, as the rear camera has limited field-of-view. At the same time, it's constrained to the robot kinematics. 
Meanwhile, the decoupled facing direction and human trajectory brings extra challenge.
We will discuss this limitation and potential solution in detail in our supplementary material (paper version). We want to clarify that this controller design is challenging and can be a separate research topic, which we leave for future work.



